Theory coherent shrinkage of Time-Varying Parameters in VARs

This paper introduces a novel theory-coherent shrinkage prior for Time-Varying Parameter VARs (TVP-VARs). The prior centers the time-varying parameters on a path implied a priori by an underlying economic theory, chosen to describe the dynamics of the macroeconomic variables in the system. Leveraging information from conventional economic theory using this prior significantly improves inference precision and forecast accuracy compared to the standard TVP-VAR. In an application, I use this prior to incorporate information from a New Keynesian model that includes both the Zero Lower Bound (ZLB) and forward guidance into a medium-scale TVP-VAR model. This approach leads to more precise estimates of the impulse response functions, revealing a distinct propagation of risk premium shocks inside and outside the ZLB in US data.

==> notes.tex <==
\subsection{Theory coherent shrinkage of time varying parameters}
Suppose that we have $\gamma$ observations from a more tightly parameterized state space model (DSGE). The likelihood of the $\gamma$ observations is: 

\begin{equation}
\begin{aligned}
p(\boldsymbol{y_t}|\boldsymbol{\Phi,\Sigma}) & = \prod_{t = 1}^{\gamma}\left(\frac{1}{2\pi}\right)^{\frac{N}{2}}| \boldsymbol{\Sigma}|^{-\frac{1}{2}}exp \left[-\frac{1}{2}\left(\boldsymbol{y}_t - \boldsymbol{x_t\Phi_t} \right)'\boldsymbol{\Sigma}^{-1}\left(\boldsymbol{y}_t - \boldsymbol{x_t\Phi_t} \right) \right] \\
\end{aligned}
\end{equation}
In compact form is: 
\[
\begin{aligned} 
L(\boldsymbol{Y^*}|\boldsymbol{\Sigma, \Phi})  & =  (2\pi)^{-\frac{\gamma N}{2}}|\boldsymbol{ \Sigma}|^{-\frac{\gamma}{2}} exp \left[-\frac{1}{2}tr( \left(\boldsymbol{\Sigma}^{-1})(\boldsymbol{Y^*} - \boldsymbol{X^*}\boldsymbol{\Phi})'(\boldsymbol{Y^*} - \boldsymbol{X^*\Phi})\right)  \right] \\
& =  (2\pi)^{-\frac{\gamma N}{2}}|\boldsymbol{ \Sigma}|^{-\frac{\gamma}{2}} exp \left[-\frac{1}{2}tr( \left(\boldsymbol{\Sigma}^{-1})(\boldsymbol{Y^*'Y^*} - \boldsymbol{\Phi}' \boldsymbol{X^*}'\boldsymbol{Y^*} - \boldsymbol{Y^*}'\boldsymbol{X^*}\boldsymbol{\Phi} + \boldsymbol{\Phi}\boldsymbol{X^*}'\boldsymbol{X^*}\boldsymbol{\Phi})\right)  \right] \\
%& =  (2\pi)^{-\frac{\gamma N}{2}}|\boldsymbol{ \Sigma}|^{-\frac{\gamma}{2}} exp \left[-\frac{1}{2}tr\left(( \boldsymbol{\Sigma}^{-1})(\boldsymbol{Y^*}'\boldsymbol{Y^*}  - \boldsymbol{Y^*'X^*(X^*'X^*)^{-1}X^*'Y^*})\right)   -\frac{1}{2}tr \left((\boldsymbol{\Sigma}^{-1})(\boldsymbol{\Phi - \hat{\Phi}})'\boldsymbol{X^*'X^*}(\boldsymbol{\Phi - \hat{\Phi}})\right)  \right]
\end{aligned}
\]
%where $\boldsymbol{\hat{\Phi}^*} = \boldsymbol{({X^*'X^*})^{-1}X^*'Y^*}$. 


Suppose that we have the moments of the state space model in closed form, as a function of some hyper-parameters $\boldsymbol{\theta}$. Staking the moments in the matrices $\boldsymbol{\Gamma_{xx}}$,  $\boldsymbol{\Gamma_{xy}}$,
and $\boldsymbol{\Gamma_{yy}}$
we can substitute  $\boldsymbol{X^*'X^*}$
$\boldsymbol{Y^*'Y^*}$,  $\boldsymbol{X^*'Y^*}$ with the state space theoretical population moments: 

\[
\begin{aligned} 
L(\boldsymbol{Y^*}|\boldsymbol{\Sigma, \Phi}) = &  (2\pi)^{-\frac{\gamma N}{2}}|\boldsymbol{ \Sigma}|^{-\frac{\gamma}{2}} exp \left[-\frac{1}{2}tr( \left(\boldsymbol{\Sigma}^{-1})(\boldsymbol{\Gamma_{yy}}  - \boldsymbol{\Phi}' \boldsymbol{\Gamma_{xy}} - \boldsymbol{\Gamma_{yx}}\boldsymbol{\Phi} + \boldsymbol{\Phi}\boldsymbol{\Gamma_{xx}}\boldsymbol{\Phi})\right)  \right] 
%& (2\pi)^{-\frac{\gamma N}{2}}|\boldsymbol{ \Sigma}|^{-\frac{\gamma}{2}} exp \left[-\frac{1}{2}tr\left(( \boldsymbol{\Sigma}^{-1})(\boldsymbol{\Gamma_{yy}}  +  \boldsymbol{\Gamma_{yx}\Gamma_{xx}^{-1}\Gamma_{xy}})\right) \right]
%=  (2\pi)^{-\frac{\gamma N}{2}}|\boldsymbol{ \Sigma}|^{-\frac{\gamma}{2}} exp \left[-\frac{1}{2}tr\left(( \boldsymbol{\Sigma}^{-1})(\boldsymbol{\Gamma_{yy}}  - \boldsymbol{\Gamma_{yx}\Gamma_{xx}^{-1}\Gamma_{xy}})\right)   -\frac{1}{2}tr \left((\boldsymbol{\Sigma}^{-1})(\boldsymbol{\Phi - \hat{\Phi}^*})'\boldsymbol{\Gamma_{xx}}(\boldsymbol{\Phi - \hat{\Phi}^*})\right)  
\end{aligned}
\]


%where $\boldsymbol{\hat{\Phi}^*} = \boldsymbol{\Gamma_{xx}^{-1}\Gamma_{xy}}$. Combining with: 


\[
\begin{aligned}
 p(\boldsymbol{\Sigma}, \boldsymbol{\Phi}|\boldsymbol{\Lambda}) & =  (2\pi)^{-\frac{TkN}{2}}|\boldsymbol{\Sigma} \otimes (\boldsymbol{H_{Tk}'H_{Tk}( I_T \otimes \Lambda'\Lambda)})^{-1} |^{-\frac{T}{2}} exp \left[  -\frac{1}{2}tr \left((\boldsymbol{\Sigma}^{-1})(\boldsymbol{\Phi - \underline{\Phi_0}})'(\boldsymbol{H_{Tk}'H_{Tk}( I_T \otimes \Lambda'\Lambda)})(\boldsymbol{\Phi - \underline{\Phi_0}})\right)  \right] \\
 & \times \frac{|\boldsymbol{\underline{S}}|^{\boldsymbol{\underline{\nu}}/2}}{2^{\boldsymbol{\underline{\nu} N}/2}\Gamma_n \left( \frac{\underline{\nu}}{2} \right)} |\boldsymbol{\Sigma}|^{-\frac{(\underline{\nu} + N+1)}{2}} exp \left[-\frac{1}{2}tr(\boldsymbol{\underline{S}}\boldsymbol{\Sigma^{-1}} ) \right]   
\end{aligned}
\]

leads to:

\[ 
\begin{aligned} 
vec(\boldsymbol{\Phi}| \boldsymbol{\Sigma}) & \sim \mathcal{N}\left( vec( \left(\gamma\boldsymbol{\Gamma_{xx}(\theta)} + \boldsymbol{H_{Tk}'H_{Tk}(I_T \otimes \Lambda'\Lambda})\right)^{-1}( \gamma\boldsymbol{\Gamma_{xy}(\theta)} + \boldsymbol{H}_{Tk}'\boldsymbol{H}_{Tk}(\boldsymbol{I_T \otimes \Lambda'\Lambda})\boldsymbol{\underline{\Phi_{0}}} )), \boldsymbol{\Sigma} \otimes (\gamma\boldsymbol{\Gamma_{xx}(\theta)}  +  \boldsymbol{H_{Tk}'H_{Tk}(I_T \otimes \Lambda'\Lambda}))^{-1}   \right) \\
p(\boldsymbol{\Sigma}) & \sim IW(\underline{S} + \gamma \boldsymbol{\Gamma_{yy}(\theta)} +   \boldsymbol{\underline{\Phi_{0}}}'(\boldsymbol{H_{Tk}}' \boldsymbol{H_{Tk}})(\boldsymbol{I_T} \otimes \boldsymbol{\Lambda'\Lambda})\boldsymbol{\underline{\Phi_{0}}} - \boldsymbol{\tilde{\Phi}}'\boldsymbol{\tilde{\Psi}}^{-1}\boldsymbol{\tilde{\Phi}} ,\underline{\nu} + \gamma)
\end{aligned}
\]
\normalsize

Assuming $\lambda_i = \lambda$ for $i = 1, \ldots, k$, we have: 

\[ 
\begin{aligned} 
vec(\boldsymbol{\Phi}| \boldsymbol{\Sigma}) & \sim \mathcal{N}\left( vec( \left(\gamma\boldsymbol{\Gamma_{xx}(\theta)} + \lambda^2\boldsymbol{H_{Tk}'H_{Tk}}\right)^{-1}( \gamma\boldsymbol{\Gamma_{xy}(\theta)} + \lambda^2\boldsymbol{H}_{Tk}'\boldsymbol{H}_{Tk}\boldsymbol{\underline{\Phi_{0}}} )), \boldsymbol{\Sigma} \otimes (\gamma\boldsymbol{\Gamma_{xx}(\theta)}  +  \lambda^2\boldsymbol{H_{Tk}'H_{Tk}})^{-1}   \right) \\
\end{aligned}
\]


\[ 
\begin{aligned} 
p(\boldsymbol{\Sigma}) & \sim IW(\underline{S} + \gamma \boldsymbol{\Gamma_{yy}(\theta)} +   \lambda^2\boldsymbol{\underline{\Phi_{0}}}'(\boldsymbol{H_{Tk}}' \boldsymbol{H_{Tk}})\boldsymbol{\underline{\Phi_{0}}} - \boldsymbol{\tilde{\Phi}}'\boldsymbol{\tilde{\Psi}}^{-1}\boldsymbol{\tilde{\Phi}} ,\underline{\nu} + \gamma)
\end{aligned}
\]

Our objective is to draw from $p(\boldsymbol{\Phi, \Sigma, \Lambda}|\boldsymbol{y})$,  that is: 

%{2}}|\boldsymbol{ \Sigma}|^{-\frac{T}{2}} exp \left[-\frac{1}{2}tr\left(( \boldsymbol{\Sigma}^{-1})(\boldsymbol{Y}'\boldsymbol{Y}  - \boldsymbol{Y'X(X'X)^{-1}X'Y})\right)   -\frac{1}{2}tr \left((\boldsymbol{\Sigma}^{-1})(\boldsymbol{\Phi - \hat{\Phi}})'\boldsymbol{X'X}(\boldsymbol{\Phi - \hat{\Phi}})\right)  \right]  \\
\[
\begin{aligned}
p(\boldsymbol{\Phi, \Sigma, \Lambda}|\boldsymbol{y}) & =  (2\pi)^{-\frac{TN}{2}}|\boldsymbol{ \Sigma}|^{-\frac{T}{2}} exp \left[-\frac{1}{2}tr\left(( \boldsymbol{\Sigma}^{-1})(\boldsymbol{Y} - \boldsymbol{X\Phi})'(\boldsymbol{Y} - \boldsymbol{X\Phi}))\right)  \right]  \\
& \times (2\pi)^{-\frac{TkN}{2}}|\boldsymbol{\Sigma} \otimes (\boldsymbol{H_{Tk}'H_{Tk}( I_T \otimes \Lambda'\Lambda)})^{-1} |^{-\frac{1}{2}} exp \left[  -\frac{1}{2}tr \left((\boldsymbol{\Sigma}^{-1})(\boldsymbol{\Phi - \underline{\Phi_0}})'(\boldsymbol{H_{Tk}'H_{Tk}( I_T \otimes \Lambda'\Lambda)})(\boldsymbol{\Phi - \underline{\Phi_0}})\right)  \right]  \\
& \times \frac{|\boldsymbol{\underline{S}}|^{\boldsymbol{\underline{\nu}}/2}}{2^{\boldsymbol{\underline{\nu} N}/2}\Gamma_n \left( \frac{\underline{\nu}}{2} \right)} |\boldsymbol{\Sigma}|^{-\frac{(\underline{\nu} + N+1)}{2}} exp \left[-\frac{1}{2}tr(\boldsymbol{\underline{S}}\boldsymbol{\Sigma^{-1}} ) \right]\\
& \times p(\boldsymbol{\Lambda})  \\
\end{aligned}
\]
%%%%%%%%%%%%%%

small scale

%
\fi



==> setup_slides.tex <==

%% UPLOAD PACKAGES
%\usepackage[beamer]{hf-tikz}



